Collective Phenomena in the Non-Equilibrium Quark-Gluon Plasma

In this work we study the non-equilibrium dynamics of a quark-gluon plasma, as created in heavy-ion collisions. We investigate how big of a role plasma instabilities can play in the isotropization and equilibration of a quark-gluon plasma. In particular, we determine, among other things, how much collisions between the particles can reduce the growth rate of unstable modes. This is done both in a model calculation using the hard-loop approximation, as well as in a real-time lattice simulation combining both classical Yang-Mills-fields as well as inter-particle collisions. The new extended version of the simulation is also used to investigate jet transport in isotropic media, leading to a cutoff-independent result for the transport coefficient q-hat. The precise determination of such transport coefficients is essential, since they can provide important information about the medium created in heavy-ion collisions. In anisotropic media, the effect of instabilities on jet transport is studied, leading to a possible explanation for the experimental observation that high-energy jets traversing the plasma perpendicular to the beam axis experience much stronger broadening in rapidity than in azimuth. The investigation of collective modes in the hard-loop limit is extended to fermionic modes, which are shown to be all stable. Finally, we study the possibility of using high energy photon production as a tool to experimentally determine the anisotropy of the created system. Knowledge of the degree of local momentum-space anisotropy reached in a heavy-ion collision is essential for the study of instabilities and their role for isotropization and thermalization, because their growth rate depends strongly on the anisotropy

==> introdraft.tex <==
qcd - history
hics - history
qgp - what is it
collective effects/instabilities
parton cascades ->now with collective effects
outline


==> jets.tex <==
\chapter{Jet broadening in unstable non-Abelian plasmas}
\label{jetunstable}
In heavy ion collisions, locally anisotropic momentum distributions
may emerge due to the longitudinal expansion. Such anisotropies
generically give rise to instabilities~\cite{Romatschke:2003ms};
see~\cite{Dumitru:2005gp,Dumitru:2006pz} for simulations of unstable
non-Abelian plasmas within the present ``Wong-Yang-Mills'' approach.
Here, we investigate their effect on the momentum broadening of jets,
including the effect of collisions.  The initial momentum distribution
for the hard plasma gluons is taken to be
\begin{align}
\label{anisof}
f(\mathbf{p})=n_g \left(\frac{2\pi}{p_{\text{h}}}\right)^2 \delta(p_z)
  \exp(-p_\perp/p_{\text{h}})\,, 
\end{align}
with $p_\perp=\sqrt{p_x^2+p_y^2}$. This represents a quasi-thermal
distribution in two dimensions with average momentum $=2\,p_{\text{h}}$.
We initialize small-amplitude fields sampled from a
Gaussian distribution and set $k^*\approx p_{\text{h}}$, for the
reasons alluded to above. The band of unstable modes is located below
$k^*$.

We find that binary collisions among hard particles reduce the growth
rate of unstable field modes, in agreement with
expectations~\cite{Schenke:2006xu}. However, for
$p_{\text{h}}=16$~GeV, $L=5$~fm, $n_g=10/\text{fm}^3$, $g=2$,
$m_\infty\simeq1$/fm and $k^*\approx p_{\text{h}}$, the reduction of
the growth rate is less than $15\%$, increasing to about $40\%$ when
$k^*\approx p_{\text{h}}/2$. This is due to fewer available field
modes and more randomizing collisions.

Next, we add additional high momentum particles with $p_x=12\,
p_{\text{h}}$ and $p_x=6\, p_{\text{h}}$, respectively, to investigate
the broadening in the $y$ and $z$ directions via the variances
\begin{align}
	\kappa_\perp(p_x):=\frac{d}{dt}\langle(\Delta
        p_\perp)^2\rangle\,, 
      ~~~\kappa_z(p_x):=\frac{d}{dt}\langle(\Delta p_z)^2\rangle\,.
\end{align}
The ratio $\kappa_z/\kappa_\perp$ can be roughly associated with the
ratio of jet correlation widths in azimuth and rapidity:
${\kappa_z}/{\kappa_\perp} \approx {\langle\Delta\eta\rangle} /
{\langle\Delta\phi\rangle}$. Experimental data on dihadron
correlation functions for central Au+Au collisions at
$\sqrt{s}=200$~GeV~\cite{Jacobs:2005pk} are consistent with
$\kappa_z/\kappa_\perp\approx 3$~\cite{Romatschke:2006bb}.  Photon-jet
correlation measurements should provide additional insight in the
future.

\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=12cm]{figures/pxyjet192lines}
    \caption{(Color online) Momentum broadening of a jet in the
      directions transverse to its initial momentum. $p_z$ is directed
      along the beam axis, $p_\perp$ is transverse to the
      beam. Anisotropic plasma, $64^3$ lattice.}
    \label{fig:pxyjet192}
  \end{center}
\end{figure}
Fig.~\ref{fig:pxyjet192} shows the time evolution of $\langle
p_\perp^2 \rangle$ and of $\langle p_z^2 \rangle$. The strong growth
of the soft fields sets in at about $t\simeq 10 \,m_\infty^{-1}$ and
saturates around $t\simeq 25\, m_\infty^{-1}$ due to the finite lattice
spacing (also see \cite{Dumitru:2006pz}). Outside of the above time
interval the ratio $\kappa_z/\kappa_\perp\approx1$.
During the period of instability, however,
\begin{align}
	\frac{\kappa_z}{\kappa_\perp} \approx 2.3\,,
\end{align}
for both jet energies shown in Fig.~\ref{fig:pxyjet192}.  We find
approximately the same ratio for denser plasmas ($n_g=20/\text{fm}^3$
and $n_g=40/\text{fm}^3$). Reducing the number of lattice sites and
scaling $p_{\text{h}}$ down to 8~GeV gives
$\kappa_z/\kappa_\perp\approx2.1$. However, these latter runs are
rather far from the continuum limit and lattice artifacts are
significant~\cite{Dumitru:2006pz}.

Initially $\xi\equiv \langle p_\perp^2\rangle /\langle p_z^2\rangle$
is infinite. However, due to collisions and the backreaction of the
fields on the hard particles we find that $\xi\approx 20$ at $t
\approx 20\, m_\infty^{-1}$.  This puts our measured ratio for
$\kappa_z/\kappa_\perp$ in the same range as those calculated
in~\cite{Romatschke:2006bb} for heavy quarks to leading-log accuracy,
where $\kappa_z/\kappa_\perp\simeq3.6$ was obtained for $\xi=10$ and
velocity $v=0.95$. We emphasize that all of these estimates apply to
the early pre-equilibrium stage before hydrodynamic evolution sets in.

The explanation for the larger broadening along the beam axis is as
follows. In the Abelian case the instability generates predominantly
transverse magnetic fields which deflect the particles in
the $z$-direction~\cite{Majumder:2006wi}.

\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=12cm]{figures/ratio-av}
    \caption{(Color online) Ratios of fourier transforms of the field energy
      densities (integrated over $k_z$) at various times; the gauge
      potentials were transformed to Coulomb gauge.}
    \label{fig:FTs}
  \end{center}
\end{figure}
In the non-Abelian case, however, on three-dimensional lattices
transverse magnetic fields are much less dominant (see, e.g.\ Fig.~5
in~\cite{Dumitru:2006pz}) although they do form larger coherent
domains in the transverse plane at intermediate times than $E_\perp$,
Fig.~\ref{fig:FTs}. Longitudinal fields and locally non-zero
Chern-Simons number $\sim {\rm tr}~\mathbf{E} \cdot \mathbf{B}$
emerge, also. Nevertheless, Fig.~\ref{fig:ratios} shows that
$E_z>B_z$, aside from $B_\perp>E_\perp$.  Hence, the field
configurations are such that particles are deflected preferentially in
the longitudinal $z$-direction (to restore isotropy).
\begin{figure}[htb]
  \begin{center}
    \includegraphics[width=12cm]{figures/ratio-tz}
    \caption{(Color online) Ratios of field energy densities.}
    \label{fig:ratios}
  \end{center}
\end{figure}

A third contribution to $p_z$ broadening in an expanding plasma, not
considered explicitly here, is due to a longitudinal collective flow
field which ``blows'' the jet fragments to the
side~\cite{Armesto:2004vz}. This mechanism is also available for
collision dominated plasmas with (nearly) isotropic momentum
distribution. However, rather strong flow gradients seem to be
required to reproduce the observed broadening of midrapidity jets (the
flow velocity has to vary substantially {\em within} the narrow jet
cone). In contrast, color fields will naturally deflect particles with
lower momentum by larger angles ($\Delta p\sim E,B$): the jet profile
broadens even if the induced radiation is exactly collinear. It is
therefore important to determine, experimentally, whether the
asymmetric broadening is related to the {\em macroscopic} collective
flow or to an anisotropy of the plasma in the local rest frame.





==> scales.tex <==
\chapter{Scales}
\label{appscales} We discuss the orders of the soft fields as well
as that of the fluctuations of the hard particles.

